Find a Way Forward: a Language-Guided Semantic Map Navigator

In this paper, we introduce the map-language navigation task where an agent executes natural language instructions and moves to the target position based only on a given 3D semantic map. To tackle the task, we design the instruction-aware Path Proposal and Discrimination model (iPPD). Our approach leverages map information to provide instruction-aware path proposals, i.e., it selects all potential instruction-aligned candidate paths to reduce the solution space. Next, to represent the map observations along a path for a better modality alignment, a novel Path Feature Encoding scheme tailored for semantic maps is proposed. An attention-based Language Driven Discriminator is designed to evaluate path candidates and determine the best path as the final result. Our method can naturally avoid error accumulation compared with single-step greedy decision methods. Comparing to a single-step imitation learning approach, iPPD has performance gains above 17% on navigation success and 0.18 on path matching measurement nDTW in challenging unseen environments.

==> 5_conclusion.tex <==
\section{limitation and future work}
%Although our proposed algorithm achieves good performance in seen environments for both success rate and nDTW, its success rate in unseen environments is still inadequate. 
So far, we can only deal with stationary environments. 
%
Dynamic objects need to be dealt with separately to avoid collision with them. 
Some obstacle avoidance mechanism may need to be introduced down the road.
In our setting, we assume the instruction corresponds to a shortest path between two points. 
%
If an instruction requires a detour, the path candidates may not be the best fit.

%Further investigating how to improve the algorithm's performance in unseen environment while also maintaining its good performance in seen environment, 
%Improving the endpoint prediction in unseen environment might require extra local information provided from RGBD sensor, since there is no description to supplement the missing concepts of semantic maps. 
% We assume this is due to a smaller dataset size and lack of a pretraining strategy for the map modality. Further investigations such as
To further improve our methods, we consider the following future works: 
(a)  Large-scale pretraining has gained a large success in the computer vision~\cite{dosovitskiy2020image} and natural language processing communities~\cite{devlin2018bert} by showing powerful generalization. Developing pretraining strategies for semantic navigation maps might increase the adaptation ability of the map-language navigator in more diverse environments.
(b) Our current auto-generated dataset only contains complete single-floor environments, we propose to design and construct a larger and semantic meaningful dataset on multi-floor environments.
(c) Designing path pruning strategies conditioned on natural language instructions is a promising direction to move forward. It has the potential to be combined with neural-symbolic models ~\cite{mao2019neuro}.

% such as traiBning the model with more dataset, using pretrained model to encode path feature or designing better language representation, would be meaningful future works.

In addition, our algorithm is able to provide multiple candidate paths based on a ranking score, which is a good feature for human-robot interaction. When the agent feels confused about vague instructions, our method provides opportunities to include additional constraints from a human. In other words, it would be interesting to study how the agent could ask the human for further explanation and clarification. Such an approach would benefit research topics such as embodied question answering and embodied dialog.

% Our algorithm plans and scores multiple paths for each instruction, which makes it easy to detect if the model feel confused about the instruction where several different paths would have similar high score. It would also be interesting to study how to endow our model the ability of asking questions back to human to clarify the ambiguity in the instruction when it gets confused. 

\section{Conclusion}

We propose a novel approach % a novel technical route 
to deal with a map-language guided navigation task. 
%
The strategy of dividing the navigation problem into three sub-problems provides a new and successful perspective for solving the problem. 
%
The deterministic path proposal scheme can leverage the global information of the maps well and reformulates the original task into a new one whose solution space is reduced, which greatly avoids accumulating errors and falling into local solutions. 
%
Our path feature embedding enables the navigator to perceive the environments from semantic navigation maps, and it can make great use of the map information compared to methods that naively use convolutional layers for feature extraction. 
%
With the designed score metric, Language Driven Discriminator can learn the alignment between modalities from the supervision. The discriminator has the capability to distinguish paths that match natural language instructions.    

Extensive experiments demonstrate the superiority of our method, especially in long distance navigation and training efficiency. 
%
Even though having some points for improvement, this propose-and-discriminate scheme has the potential to be a promising direction.

%planning plus learning is a worthy approach for dealing with language-guided navigation on semantic maps.
%The effectiveness and efficiency of introducing an advanced planning method into a deep learning framework should be further explored. We have observed that a detailed description of the local environment cannot be effectively handled when only modeled by semantic maps, so we leave the study of introducing RGBD image information in order to improve the local planning to future work.






% \newpage

% \begin{table*}
%  \centering
%     \begin{threeparttable}
%         \begin{tabular}{ c cccccc cccccc } 
%         \toprule
%          \multirow{2}{*}{\textbf{\# Attention Layer}} & \multicolumn{6}{c}{\textbf{Val-Seen} } & \multicolumn{6}{c}{\textbf{Val-Unseen} }\\
%          \cmidrule(lr{1em}){2-7}  \cmidrule(lr{1em}){8-13} 
%         & TL & NE & nDTW & OS & SR & SPL &  TL & DG & nDTW & OS & SR & SPL  \\
%         \midrule
%         \textbf{1} &  8.55 & 8.59 & 0.48 & 0.34 & 25.6 & 0.24 & 7.57 & 6.83 & 0.54 & 0.34 & 22.6 & 0.21\\

%         \textbf{2} & 8.24 & 7.63 & 0.54 & 0.38 & 31.3 & 0.31 & 7.00 & 6.48 & 0.55 & 0.36 & 21.9 & 0.20\\

%          \textbf{3} &  8.36 & 7.68 & 0.54 & 0.37 & 32.1 & 0.31 & 6.99 & 5.99 & 0.57 & 0.33 & 22.4 & 0.21 \\
     
%          \textbf{4} & 8.36 & 7.71 & 0.53 & 0.38 & 32.5 & 0.32 & 7.40 & 5.87 & 0.58 & 0.37 & 23.8 & 0.23  \\

%          \textbf{5} & 8.23 & 7.52 & 0.54 & 0.41 & 34.1 & 0.33 & 7.04 & 5.93 & 0.57 & 0.32 & 22.1 & 0.22 \\
         
%          \textbf{6} & 8.25 & 6.99 & 0.57 & 0.44 & 38.2 & 0.37 & 6.81 & 5.65 & 0.58 & 0.35 & 24.0 & 0.23 \\
         
%         \bottomrule
%         \end{tabular}
%     \end{threeparttable}
%     \vspace{-1ex}
%     \caption{Influence of number of transformer layers }
%     \label{Ablation study}
%     \vspace{-2ex}
% \end{table*}
